Astraea: Grammar-based Fairness Testing

Software often produces biased outputs. In particular, machine learning (ML) based software are known to produce erroneous predictions when processing discriminatory inputs. Such unfair program behavior can be caused by societal bias. In the last few years, Amazon, Microsoft and Google have provided software services that produce unfair outputs, mostly due to societal bias (e.g. gender or race). In such events, developers are saddled with the task of conducting fairness testing. Fairness testing is challenging; developers are tasked with generating discriminatory inputs that reveal and explain biases. We propose a grammar-based fairness testing approach (called ASTRAEA) which leverages context-free grammars to generate discriminatory inputs that reveal fairness violations in software systems. Using probabilistic grammars, ASTRAEA also provides fault diagnosis by isolating the cause of observed software bias. ASTRAEA's diagnoses facilitate the improvement of ML fairness. ASTRAEA was evaluated on 18 software systems that provide three major natural language processing (NLP) services. In our evaluation, ASTRAEA generated fairness violations with a rate of ~18%. ASTRAEA generated over 573K discriminatory test cases and found over 102K fairness violations. Furthermore, ASTRAEA improves software fairness by ~76%, via model-retraining.

==> response.tex <==
\section*{Minor Revision Response for "Astraea: Grammar-based Fairness Testing"}
\label{sec:intro}

%\todo{Thank editor}

%\revise{
We would like to thank the associate editor and reviewers for their insightful comments, we appreciate the reviewers efforts in helping us improve our paper. We have addressed all reviewer comments in the paper. In the following, we respond to each comment or issue raised and refer the reviewer to where to find them in the revised paper. Kindly note that all texts marks in color {\textcolor{blue}{blue}} in the paper are newly added or modified portions to address the issues raised in the reviews. 
%}


\section*{Associate Editor Comments}
\label{sec:overview-ae}
\textit{\textbf {Comment \#1:}}
Thank you for submitting to TSE and I am sorry that the review took 
longer than usual.  However, I am excited to report that the paper is 
very close to being accepted at this point.  Please take a look at the 
reviewers' comments, particularly the related work mentions, and 
prepare a minor revision.  As one of the reviewers suggests, if you 
wanted to move some of the raw data (e.g., tables 5 and 7) to 
supplementary materials, that would be fine (though that decision is up 
to you).



\smallskip \noindent
%\todo{
\textit{\textbf{Response \#1:}} 
Thank you for the insightful meta-review. We have addressed all concerns raised in the reviews in the response (”review comments”) below. Specifically, we summarize the major changes made in the revised version of the paper:

\begin{itemize}
\item \textbf{Recent Related Work:} We thank the reviewer for pointing out recent publications in fairness testing. We have added the missing papers to \Cref{sec:related-work}.
\item \textbf{Bias-related Harms:} In accordance to the reviewer comments, we have shed more light on the tangible harms of biases in Ml software. We added this in \Cref{sec:background}. 
\item \textbf{Embedding-based Debiasing:} We have added more recent work on embedding-based debiasing, especially work that handle the debiasing of contextual embeddings~\cite{dev2020measuring}. We have discussed this line of work in \Cref{sec:related-work}. 
\item \textbf{Fairness Definition:} Following the comment of the reviewer, we have discussed the definition of fairness (violation) employed in this work. We have addressed this in \Cref{sec:definitionOfTerms}.
\item \textbf{Table Placement:} Due to the importance of \autoref{tab:results-summary-ind-fairness} and \autoref{tab:gen-of-repair}, we have decided to leave them in the paper and not in the supplementary material. 
\end{itemize}

%\revise{ Thank you for the insightful meta-review. 
%We address all concerns raised in the reviews and answer all questions in the paper and in the response (''review comments'') below.
%}

\section*{Review Comments}

%\revise{
In this section, we will go through the reviewer comments and outline 
how these comments and concerns were addressed in the revised paper.
%}

\subsection*{Response for Reviewer \#1}
\smallskip \noindent 
\textit{\textbf {Comment \#1:}}
Thanks for acknowledging all the concerns. Now the paper is in much better shape than it was before. Some recent SE fairness works are missing. Please add them.
\begin{itemize}
	\item [] https://dl.acm.org/doi/10.1145/3468264.3468565,
	\item [] https://dl.acm.org/doi/10.1145/3468264.3468537,
	\item [] https://dl.acm.org/doi/10.1145/3468264.3468536
\end{itemize}

\smallskip \noindent %\todo{
\textit{\textbf{Response \#1:}}
Thank you for pointing out the following recent SE fairness works, we have addressed this by discussing them in the ``Related Work'' (\Cref{sec:related-work}), which can be seen below:

\reviseNew{
More recently,  Biswas and Rajan~\cite{fairPreprocessing} proposed a causal method to reason about the fairness impact of data preprocessing stages in the ML pipeline. Chakraborty et al.~\cite{chakraborty2021bias} proposed a mutation-based algorithm (called Fair-SMOTE) for removing biased labels and re-balancing internal distributions of sensitive attributes in ML systems, such that examples are equal in both positive and negative classes.
Besides, Hort et al.~\cite{hort2021fairea} proposed a model behaviour mutation technique to benchmark ML bias mitigation methods. 
} 


%}

\subsection*{Response for Reviewer \#2}

\smallskip \noindent 
\textit{\textbf {Comment \#1:}}
The updates to the earlier comments are great.
I would emphasize again to elaborating the segment on embedding based debiasing to explain why that hasn't been considered as a part of your pipeline. You are still citing very old papers whereas a lot of new work proves that Gonen and Goldberg's claim (that you cite) on residual bias is can be conquered with better techniques.
While the testing is sound, fairness in NLP requires a deeper exploration in the paper.


\smallskip \noindent %\todo{
\textit{\textbf{Response \#1:}}
Thank you for the insightful comment, we have addressed this concern in the ``Related Work'' section by adding recent works~\cite{dev2019attenuating,dev2020measuring}. Kindly find the discussion in \Cref{sec:related-work} and below:

\reviseNew{
Following Gonen and Goldberg~\cite{lipstick-debiasing-cover},  there has been significant work to improve existing word debiasing techniques~\cite{debiasing-word-embedings}. Notably, Dev and Phillips~\cite{dev2019attenuating} proposed a natural language inference-driven method for debiasing word embeddings. The authors further demonstrate that this approach effectively
mitigates the effect of specific biases in word embedding~\cite{dev2020measuring}. 
While these works are focused on alleviating the biases at the word embedding level, our approach complements these works. In particular, it considers the NLP model as a black box and automatically discovers biases in the model. 
%directly in NLP tasks. 
Indeed, a parallel line of  work points out the need to employ various metrics to quantify and measure %for the evaluation of 
bias in NLP systems~\cite{blodgett2021sociolinguistically}. 
This further emphasizes the need 
for a tool like \NLT to support the accurate detection
and measurement of fairness violations through systematic testing.}



\smallskip \noindent 
\textit{\textbf {Comment \#2:}}
In the discussion and description of bias, linking it to tangible harms is important. In NLP literature, it has been established that fairness testing or debiasing needs to be discussed with harms in context. Providing intuition of harms prevented or possible is important for the significance of the tool.

\smallskip \noindent %\todo{
\textit{\textbf{Response \#2:}}
Thank you for the comments, we have clarified this concern in the ``Background'' (\Cref{sec:background}), also kindly find the discussion below:

\smallskip \noindent
\reviseNew{\textbf{Bias-related Harms:} %caused by Bias in NLP Systems:} 
Bias in machine learning software generally causes 
two types of tangible harms: {\em allocative} harms and 
{\em representational} harms~\cite{crawford2017trouble}. 
On one hand, an \textit{allocative harm} is when a system withholds an 
opportunity or a resource from certain groups (e.g., women) in comparison to other groups (e.g., men). This harm is often immediate and generally easy to quantify. It has been demonstrated that ML applications
such as credit rating systems~\cite{aequitas} and risk recommendation systems~\cite{compas} may cause allocative harms. For instance, consider the COMPAS risk recommendation system for recidivism. This system exhibits an 
%For instance, an 
allocative harm 
%is exhibited by a risk recommendation system (e.g., COMPAS~\cite{compas}) system 
when it withholds resources (i.e., social justice and freedom) for certain groups (e.g., women and black minorities), even though those groups have similar (or fewer) number of crimes or even less severe crimes than other groups (e.g., men and white majorities). 
}

\reviseNew{
On the other hand, \textit{representative harms} occur when systems reinforce the subordination of some 
groups along the lines of identity. These harms are long-term and harder 
to quantify. Our work (\NLT) aims to automate the discovery of such 
harms of representation in NLP software. \NLT
allows practitioners to discover fairness violations that reinforce certain 
stereotypes (e.g., occupational stereotypes). %s or race). 
%the use case for MLM we have 
As an example, we found such representational harms in our evaluation of MLM models. For MLM models, \NLT revealed that a ``doctor'' is more likely to be predicted as ``male'', while ``nurses'' are likely to be predicted as ``female'' (see RQ2 in \Cref{sec:results}). 
Thus %revealing that the
these models may reinforce the societal stereotypes about such occupations. %, and the subordination of certain groups (i.e., female). % We envision t
Evidently, \NLT is applicable for the automatic discovery of representational harms in NLP systems.
}

\subsection*{Response for Reviewer \#3}

\smallskip \noindent 
\textit{\textbf {Summary Comment:}}
I appreciate the authors’ efforts and changes to the paper. The paper has
substantially improved. In particular, the following three changes/additions
satisfy many of my previous concerns:
\begin{enumerate}
	\item An evaluation of the semantic validity of the generated input 
	sentences, which provides proper context for the paper's evaluation 
	and claims (RQ 8).
	
	\item Interpretation and contextualization of empirical results 
	together with an explicit discussion of limitations. Additionally, 
	the extended discussion on ethical considerations and policy
	questions (section 7.3) providesimportant context for this work and 
	its applications.
	
	\item Consistent terminology and definition of terms (section~4).
   
\end{enumerate}

\smallskip \noindent 
The statistical analysis of the empirical results remains weak (no statistical
analysis beyond the regression analysis around RQ4). That said, the claims and
discussions in the paper are now largely aligned with the reported basic
(descriptive) statistics.


\smallskip \noindent %\todo{
\textit{\textbf{Summary Response :}} Thank you for helping us improve the paper, we respond to all individual comments below. 
%}


\smallskip \noindent 
\textit{\textbf {Comment \#1:}}
Section 4 should provide a clear and direct definition of the term
 "fairness", aligned with the goals of the paper. The current definition only
 equates the terms "unfair" and "bias", but fairness itself is not defined
 (is fairness dichotomous, is it the degree to which a system is free of
 bias, or something else?). Also, I suggest to incorporate the notion of a
 policy into the definition of fairness. Finally, the paper currently defines
 individual fairness as a *violation* of the Lipschitz property [27], which
 causes additional confusion. Section 4 should clearly define fairness and
 fairness violation and then use these terms consistently throughout.


\smallskip \noindent %\todo{
\textit{\textbf{Response \#1:}} 
Thank you for pointing out this issue. 
We have clarified the definition of fairness in the ``Definition of Terms'' (\Cref{sec:definitionOfTerms}), which can be seen below:


\smallskip \noindent
\reviseNew{\textbf{Software Fairness:} }
\reviseNew{ %In this work, w
%In this paper, %e previous section, 
%we use the term {\em unfair} to describe bias. 
%There has been a significant work in understanding and defining {\em unfair} 
%behavior~\cite{verma2018fairness}. In particular, 
%w
We explore \textit{fairness as a software property}, especially in terms of \textit{software quality}~\cite{galhotra2017fairness}. We are particularly interested in the quality control of fairness properties in ML-based systems (i.e., NLP software). 
The aim is to examine \textit{how to measure and prevent bias in software via the lens of software testing and debugging}. In other words, we quantify fairness as the number of fairness violations found in the input space.
For a given input, a fairness violation occurs when a software under test does not satisfy  
a given fairness criteria. 
We discuss the fairness criteria employed in this paper %defined 
below. 
%by \NLT. 
}

\smallskip \noindent 
\textit{\textbf {Comment \#2:}}
The notion of "stronger" (theorem 2) is still confusing -- largely because
 the paper interchangeably uses the terms fairness and fairness violations.
 (Using the current terminology, "stronger" fairness means "weaker" fairness
 violation conditions and vice versa.) To avoid confusion, I suggest to
 remove the vague and confusing term "stronger" and simply state and motivate
 the subset relationship at the end of theorem 2. (Note that the motivation
 and proof for theorem 2 are already in the paper; there is no need to
 introduce yet another term.) Additionally, see my comment above about
 fairness vs. fairness violation.


\smallskip \noindent %\todo{
\textit{\textbf{Response \#2:}}
Thank you. We have clarified this by replacing the term ``stronger'' with ``stricter'', since this is a standard term used to compare logical conditions.  


\smallskip \noindent 
\textit{\textbf {Comment \#3:}}
The paper should refrain from using overly general language. For example:

\smallskip \noindent
 {\em "Clearly, in this example, the difference in BERT outcomes is clearly
 higher than the expected outcomes in both use cases, the returned BERT
 outcome does not represent either the equal distribution or the real-world
 distribution of doctors. Instead, it clearly reinforces or amplifies the
 societal bias about the occupation."}
 
 \smallskip \noindent
 The policy and expected outcome question is complex and societal norms
 differ between, e.g., individual countries and regions. The paper makes
 the above claim based on a single data point from the US. I suggest to tie
 this example (BERT outcomes) back to the notion of policy more generally.
 Using the data from the US Bureau of Labor Statistics as an example is
 perfectly reasonable, but the statement as written ("real-world distribution
 of doctors") is too general.



\smallskip \noindent %\todo{
\textit{\textbf{Response \#3:}}
Thanks, we have clarified this with respect to the US labor of statistics in \Cref{sec:background}, find the amended text below: % (Page 6). 

Clearly, in this example, the difference in BERT outcomes is clearly higher than the expected outcomes in both use cases, the returned BERT outcome does not represent either the equal distribution or the 
\reviseNew{distribution of doctors seen in the US Bureau of Labor 
Statistics~\cite{labor-stats}}.

\smallskip \noindent 
\textit{\textbf {Comment \#4:}}
Figure 10: since the paper explicitly contrasts top-5 vs. top-10, the
corresponding plots should be on the same scale to aid visual comparisons.



\smallskip \noindent %\todo{
\textit{\textbf{Response \#4:}}
Thank you, we have modified the relevant plot to the same scale (now \autoref{fig:gen-repair} in this response). 

\smallskip \noindent 
\textit{\textbf {Comment \#5:}}
There are some word/sentence duplications (e.g., section 8, “completeness”
 paragraph); this might be an artifact of highlighting textual changes.
 Another careful proof-reading pass would be advisable.

\smallskip \noindent %\todo{
\textit{\textbf{Response \#5:}}
Thank you for spotting the text duplication. We have proof-read the paper and fixed similar repetitions to the best of our ability. For instance, we have modified the sentence appropriately in \Cref{sec:threats-to-validity}, also see below:

\reviseNew{
By design, \NLT is incomplete in discovering fairness violations
%\NLT is incomplete in the exploration of fairness violations 
due to several reasons, namely (1) \textit{input grammars} -- it can only expose the biases captured in the employed input grammar, (2) \textit{lack of guarantees in testing} -- %,  the incompleteness of testing, 
in comparison to the guarantees afforded by verification, \NLT does not provide a guarantee or proof of fulfilling fairness properties and (3) \textit{finite number of generated tests} - limited number of generated inputs within a reasonable time budget.}


\smallskip \noindent 
\textit{\textbf {Comment \#6:}}
Since the paper is fairly long, the authors may want to move some of its
content (e.g., raw data such as tables 5 and 7 or the details about validation
efforts such as the newly introduced RQ8) to the supplementary material.
(Just to clarify, in contrast to the above issues, I am not necessarily
expecting the authors to make this particular change.)



\smallskip \noindent %\todo{
\textit{\textbf{Response \#6:}}
Thank you for the comment. Due to the importance of these tables (\autoref{tab:results-summary-ind-fairness} and \autoref{tab:gen-of-repair}) we have decided to leave it in the paper, and not move it to the supplementary material. 



%=============================
%
%

%\smallskip \noindent 
%\textit{\textbf {Comment \#:}}
%
%\smallskip \noindent %\todo{
%\textit{\textbf{Response \#:}}



